I/O Efficient Algorithms for Matrix Computations

We analyse some QR decomposition algorithms, and show that the I/O complexity of the tile based algorithm is asymptotically the same as that of matrix multiplication. This algorithm, we show, performs the best when the tile size is chosen so that exactly one tile fits in the main memory. We propose a constant factor improvement, as well as a new recursive cache oblivious algorithm with the same asymptotic I/O complexity. We design Hessenberg, tridiagonal, and bidiagonal reductions that use banded intermediate forms, and perform only asymptotically optimal numbers of I/Os; these are the first I/O optimal algorithms for these problems. In particular, we show that known slab based algorithms for two sided reductions all have suboptimal asymptotic I/O performances, even though they have been reported to do better than the traditional algorithms on the basis of empirical evidence. We propose new tile based variants of multishift QR and QZ algorithms that under certain conditions on the number of shifts, have better seek and I/O complexities than all known variants. We show that techniques like rescheduling of computational steps, appropriate choosing of the blocking parameters and incorporating of more matrix-matrix operations, can be used to improve the I/O and seek complexities of matrix computations.

==> conclusion.tex <==
\rhead{} \lhead{Conclusions}
\chapter{Conclusions}
We have studied some problems of matrix computations. We analysed
several known algorithms. We proposed some new algorithms too. The
analyses were carried out on the external memory model of Aggarwal
and Vitter with an intent of estimating the asymptotic I/O and
seek complexities of the algorithms.

A seek is the task of positioning the read/write head of the disk
on the data block needed next. In reality, the cost of seeking a
block will depend on the location of the block on the disk
relative to the block being read or written now. We make the
simplistic assumption that every block can be sought at the same
cost. We define the seek complexity of an algorithm as the number
of times the algorithm chooses to read or write a block that is
not physically contiguous with the block being read or written
now, thereby necessitating a seek.

The I/O complexity of an algorithm is the sum of the number of
blocks of data it moves between the two levels of memory, and its
seek complexity. In all the algorithms we have seen, the former
asymptotically dominates the latter for almost all choices of
problem parameters.  Therefore (and also because, new memory
technologies (such as flash memory) tend to make switches in data
localities cheap), in all the algorithms we designed, our attempt
has been to optimise on the net data movement.

Note that while translating our complexity bounds into real time
on a disk system of today, the data movement complexity is to be
scaled using the disk access rate, while the seek complexity using
the average of ``seek time + latency''; the latter scaling factor
is usually much larger. Also, reductions in the former are not
always concomitant with reductions in the latter, as some examples
in this thesis show.

For the problems we consider in this thesis a lower bound of
$\Omega(N^3/\sqrt{M}B)$ on blocks of data to be moved is known
~\cite{bdhs-mcla-09-new}. We demonstrate matching upper bounds for
most case. In particular, we present a new algorithm that matches
the lower bound for Hessenberg reduction.

Two ratios of interest are the data utilisation ratio defined as
the number of operations performed per element moved, and the data
locality ratio defined as the number of blocks of data moved per
seek, even though neither is a suitable performance metric.

A matrix multiplication on two $t\times t$ matrices, for
$t=O(\sqrt{M})$, reads in two $t\times t$ matrices at the cost of
$O(t^2/B)$ I/Os, and performs $O(t^3)$ operations on them. With
$t=\Theta(\sqrt{M})$, the data utilisation ratio is maximised at
$\Theta(\sqrt{M})$ operations per element moved. When
$t=\omega(\sqrt{M})$, a matrix multiplication performs $O(t^3)$
operations and $O(t^3/B\sqrt{M})$ I/Os. The data utilisation ratio
remains the same. The lower bound of on the amount of data to be
moved for matrix problems~\cite{bdhs-mcla-09-new}, sets an upper
bound of $O(\sqrt{M})$ on the data utilisation ratios of their
algorithms.

The data locality ratios of matrix transposition and
multiplication algorithms discussed in Chapter~1 are
$O(\sqrt{M}/B)$. It is not known whether algorithms of larger
ratios exist for these problems. We, however, demonstrate
algorithms for other matrix problems (for eg., QR decomposition)
with data locality ratio as high as $O(M/B)$.

The I/O performances of slab based algorithms, which are not quite
state of the art anymore, depend on the the slab widths chosen. To
get the best out of these algorithms, we find, surprisingly, that
it is not always necessary that the slabs fit in the main memory.
(See Chapter~2 on QR-decomposition, for example.) Also, for
sufficiently large matrices, with the matrix multiplications
implemented using an optimal blocked OOC algorithm, we find, the
slab based algorithm for QR decomposition runs with an I/O
complexity of $O(N^3/B\sqrt{M})$.  That means existing
implementations of slab based  algorithms may not have to be
completely redesigned (into, for example, the tile based
algorithms) for good OOC performance. If some of the elementary
matrix operations in them (for example, matrix multiplication) are
handled I/O efficiently, asymptotically optimal I/O performances
might be achievable for most inputs. While this is true for
QR-decomposition, it is not for Hessenberg reduction, as we have
shown.

